Unsupervised Quantum Anomaly Detection on Noisy Quantum Processors

Whether in fundamental physics, cybersecurity or finance, the detection of anomalies with machine learning techniques is a highly relevant and active field of research, as it potentially accelerates the discovery of novel physics or criminal activities. We provide a systematic analysis of the generalization properties of the One-Class Support Vector Machine (OCSVM) algorithm, using projected quantum kernels for a realistic dataset of the latter application. These results were both theoretically simulated and experimentally validated on trapped-ion and superconducting quantum processors, by leveraging partial state tomography to obtain precise approximations of the quantum states that are used to estimate the quantum kernels. Moreover, we analyzed both platforms respective hardware-efficient feature maps over a wide range of anomaly ratios and showed that for our financial dataset in all anomaly regimes, the quantum-enhanced OCSVMs lead to better generalization properties compared to the purely classical approach. As such our work bridges the gap between theory and practice in the noisy intermediate scale quantum (NISQ) era and paves the path towards useful quantum applications.

==> archive/hardware_benchmark_table.tex <==
\begin{table}[h]
    \centering
    \caption{Feature Map: qrbf - CX.} %Simulator variance: $(\pm 0.00209, \pm 0.01457)$ }
    \begin{tabular}{|l|c|c|} \hline
         Backend & F1-Train & F1-Test \\ \hline\hline 
         Simulator & 0.83720  & 0.77030  \\ \hline
         AQT Ibex& 0.83594 & 0.75949 \\ \hline
         IonQ Harmony & 0.84825 & 0.75949 \\ \hline
         IBM Brisbane & 0.84375 & 0.82500 \\ \hline 
         IBM Kyoto & 0.84115 & 0.81481 \\ \hline
         IBM Sherbrooke & 0.84306 & 0.82051 \\ \hline
         IBM Osaka & 0.84156 & 0.77500 \\ \hline
    \end{tabular}
    \label{tab:hardware_results_cx}
    
    \caption{Feature Map: qrbf - ECR.} %Simulator variance $(\pm 0.00298, \pm 0.01989)$}
    \begin{tabular}{|l|c|c|} \hline
         Backend & F1-Train & F1-Test \\ \hline\hline 
         Simulator &  0.85913 & 0.75345 \\ \hline
         AQT Ibex & 0.85826 & 0.77922 \\ \hline
         IonQ Harmony & 0.85863 & 0.79487 \\ \hline
         IBM Brisbane & 0.85084 & 0.84211 \\ \hline
         IBM Kyoto & 0.85344 & 0.65672 \\ \hline
         IBM Sherbrooke & 0.84525 & 0.78481 \\ \hline
         IBM Osaka & 0.83225 & 0.77922 \\ \hline
    \end{tabular}
    \label{tab:hardware_results_ecr}

    \caption{Feature Map: qrbf - RXX.} %Simulator variance $(\pm 0.00274, \pm 0.01320)$}
    \begin{tabular}{|l|c|c|} \hline
         Backend & F1-Train & F1-Test \\ \hline\hline 
        Simulator & 0.84182 & 0.79292 \\ \hline
        AQT Ibex & 0.84565 & 0.82927 \\ \hline
        IonQ Harmony & 0.83896 & 0.80488 \\ \hline
        IBM Brisbane & 0.84156 & 0.80952 \\ \hline
        IBM Kyoto & 0.85863 & 0.80488 \\ \hline
        IBM Sherbrooke & 0.84416 & 0.77500 \\ \hline
        IBM Osaka & 0.84565 & 0.79012 \\ \hline    
    \end{tabular}
    \label{tab:hardware_results_rxx}
\end{table}

==> notes.tex <==
\noindent Classical shadows have well suited properties for estimating linear functions connected to observables $O_i$ for an unknown state $\rho$:
\begin{equation}\label{eq:observable}
    o_i = \mathrm{Tr}\left[ O_i \, \rho \right]\, , 1 \le i \le M \, .
\end{equation}
The theoretical guarantees in \cite{huang_shadows} however hold for taking the median after constructing $K$ chunks of estimations 
\begin{equation}\label{eq:chunks}
    \hat{o}^{(k)}_i = \frac{1}{N} \, \sum\limits_{j=N(k-1)+1}^{N k} \, \mathrm{Tr}\left[ O_i \, \hat{\rho}_j \right]\, , 
\end{equation}
such that for the median of $\hat{o}^{(1)}_i, \hat{o}^{(2)}_i, \dots, \hat{o}^{(K)}_i$ the total of $N_\mathrm{tot}$ measurement repetitions suffice for an accuracy $\left| \hat{o}_i(N_\mathrm{tot}, K) - o_i  \right| \le \varepsilon$, where 
\begin{equation}\label{eq:N_tot}
    N_\mathrm{tot} = \mathcal{O} \left(\frac{\log(M)}{\varepsilon^2} - \max\limits_{i \le i \le M} \left|\left| O_i - \frac{\mathrm{Tr}\left[ O_i \right]}{2^n} \, \mathds{1} \right|\right|^2_\mathrm{shadow} \right) \, .
\end{equation}

\noindent In our case, where we use random Pauli measurements, the second term in Eq.\eqref{eq:N_tot} can be upper bounded by $4^{\mathrm{locality}(O)} \left|\left| O \right|\right|^2_{\infty}$. The bound is tightened furthermore, due to the fact that we are only concerned with the 1Q-RDMs and hence $\mathrm{locality}(O) = 1$. Furthermore, we want to highlight the fact, that the efficiency of the tomography depends on the chosen basis. The shadow norm term in Eq.~\eqref{eq:N_tot} is directly influenced by the chosen basis. It is possible to consider generalized measurements and improve the scaling in Eq.~\eqref{eq:N_tot} \cite{optimizationshadows}. However, our choice of basis is justified by its suitability to be implemented on the basis gate sets available on current NISQ devices. Despite the fact that positive operator-valued measurements (POVMs) can always be implemented by standard projective measurements on gate-based quantum computers (for more details see ~\cite{nielsenchuang, preskill_lecturenotes}), they require additional resources and specific circuit modules. Naimark's theorem states that any $n$-element POVM on a target system A can always be performed by projective measurements by including an ancilla system B, such that the orthonormal basis states of system B are in one-to-one correspondence with the POVM outcomes. In ~\cite{yordanov_povm}, the authors proposed a scheme that performs a $n$-element POVM by adding $(n-1)$ POVM circuit modules sequentially and increasing the system size by $\log_2(n)$ ancilla qubits. The POVM circuit modules include several multi-controlled gates, which are infeasable on current NISQ computers. However, the latter obstacle could be overcome by sophisticated compilation methods, such as variational quantum compiling ~\cite{sharma_2020} or deep reinforcement learning ~\cite{moro_2021}. \\

\noindent In the past, many implementations of $\mathcal{N}$ were deployed on IBM's quantum computers. For early examples in 2017, where the 5-qubit chip \textit{IBMQX2} \& \textit{IBMQX4} were publicly available 
\begin{equation}
    \mathcal{N} = \left\{ U_1(\lambda), R_X\left(\frac{\pi}{2}\right), \mathrm{CX}\right\} \, ,
\end{equation}
where 
\begin{equation}
    \begin{split}
    U_1(\lambda) &= \begin{pmatrix} 1 & 0 \\ 0 & e^{i \lambda} \end{pmatrix} \, , \\
    R_X\left(\frac{\pi}{2}\right) &= \frac{1}{\sqrt{2}} \begin{pmatrix}
        1 & -i \\ -i & 1
    \end{pmatrix} \, , \\
    \mathrm{CX} &= \begin{pmatrix}
        1 & 0 & 0 & 0 \\
        0 & 1 & 0 & 0 \\
        0 & 0 & 0 & 1 \\
        0 & 0 & 1 & 0 
    \end{pmatrix}\, .
    \end{split}
\end{equation}
Besides that, those devices and later superconducting devices are not fully connected. Hence for a fully-connected 5-vertex graph, there should be 20 edges, whereas those 5-qubit chips only had 6 connections. 

Over the years, different gate sets were tried and the the chips connectivity was improved. Further improvements in the control of the qubits were achieved by leveraging so-called virtual $Z$-rotations (VZ) \cite{krantz2019}. VZs realize Z-rotations without physically performing those. Instead, a corresponding phase-shift is applied to the driving signal. 

On the hardware the physical realization of CX is obtained by the so-called cross resonance gate (CR) \cite{gambetta2016, gambetta2020}, e.g. by driving qubit A with the resonance frequency of the neighbouring qubit B approximately resulting in an effective Hamiltonian with $Z \otimes X, I \otimes Z, I \otimes X, Z \otimes I, Z \otimes Z$ terms. The most important term is $Z \otimes X$, since it resembles the standard CX gate locally for a specific angle. Hence, unwanted terms such as $I \otimes Z$ need to be suppressed. This in practice is achieved by adding target rotary rotary pulses during the echoing of the CR gate. 

and equivalent to a $CX$ up to local $Z$-rotations. $R_{XX}, R_{ZZ}$ and $R_{XY}$ called M\o ller-S\o rensen (MS) gates are state-of-the-art realizations of entanglement on trapped-ion systems \cite{molmer_sorensen, molmer_sorensen_2, molmer_sorensen_3}. Originally the Cirac-Zoller CX (CZ-CX) gate was proposed in 1995 \cite{cirac_zoller} and realized in 2003 \cite{cirac_zoller_2}. However, this realization is more sensitive to errors and hence MS gates are preferred, though in theory CZ-CXs can be faster than MS gates. \\
